Safety-Guarantee Controller Synthesis for Cyber-Physical Systems

The verification and validation of cyber-physical systems is known to be a difficult problem due to the different modeling abstractions used for control components and for software components. A recent trend to address this difficulty is to reduce the need for verification by adopting correct-by-design methodologies. According to the correct-by-design paradigm, one seeks to automatically synthesize a controller that can be refined into code and that enforces temporal specifications on the cyber-physical system. In this paper we consider an instance of this problem where the specifications are given by a fragment of Linear Temporal Logic (LTL) and the physical environment is described by a smooth differential equation. The contribution of this paper is to show that synthesis for cyber-physical systems is viable by considering a fragment of LTL that is expressive enough to describe interesting properties but simple enough to avoid Safra's construction. We report on two examples illustrating a preliminary implementation of these techniques on the tool PESSOALTL.

==> controller-synthesis.tex <==
\section{Controller Synthesis}



%The decomposition property in Proposition~\ref{Prop:Decompose} allows for a compositional approach to controller synthesis. 
Algorithm~\ref{algo:synthesize} illustrates the steps we have implemented to construct the controller and the winning states of the system $S$ with respect to a given specification.
We handle the full safe-LTL set. Moreover, we support formulas of form- $\varphi_{safe} \land\varphi_{guarantee}$ where $\varphi_{safe}$ is a safe-LTL formula and 
$\varphi_{guarantee}$ is of type $\Diamond\ \gamma$ with $\gamma$ an atomic proposition.
We note that LTL formuls with $\U$ operators can be expressed in our logic, since 
$$p\ \U\ q\ =\ (p\ \W\ q)\ \land\ \Diamond r$$.
Given a formulae $\varphi_{safe}$, we can compute NNF of
$\lnot \varphi_{safe}$ by calling \emph{nnf} procedure. 
Let $\phi$ be the NNF form of $\lnot \varphi_{safe}$.
We have already described the algorithm \emph{ConstructFineAutomata} to compute the
fine automaton $A^{Fine}_{\phi,nondet}$.
The constructed non-deterministic automaton is determinized by the procedure \emph{doSubsetConstruction} into DFA $A^{Fine}_{\phi}$
Given a deterministic fine automaton with respect to $\lnot \varphi_{safe}$, and
the system $S$, the procedure \emph{computeSynchronousProduct} computes the synchronous product $P_{\phi}$.
$SolveSafety$ $Game$ computes the winning set $W$ and the controller 
transition relation $C$. 
We first synthesize a controller $C_{\varphi_{safe}}$ enforcing $\varphi_{safe}$ on the system $S$ and consider the new system $C_{\varphi_{safe}}\times S$.
The procedure also updates the winning states and transition relation of system $P$ with the winning states $W$ and controller transition relation $C$ respectively.

From Thoerem~\ref{th:fine}, we know that the $SolveSafety$ $Game$ procedure
returns a maximal strategy for the controller and we do not loose any satisfying strategies.
Since $C_{\varphi_{safe}}$ is the least restrictive controller enforcing $\varphi_{safe}$, a controller enforcing $\varphi_{safe} \land \varphi_{guarantee}$ can now be obtained as 
$ C_{\varphi_{guarantee}}$ where $C_{\varphi_{guarantee}}$ is a controller enforcing $\varphi_{guarantee}$ on $C_{\varphi_{safe}} \times S$.
The current implementation in {\sc pessoa} only handles formulas $\varphi=\psi\,\land\,\Diamond\,\gamma$ where $\gamma$ is an atomic proposition. Hence, the synthesis of a controller enforcing $\Diamond\,\gamma$ reduces to a simple reachability game with objective $\gamma$.
\emph{SolveReachabilityGame}  computes the winning set and controller transitions for this reachability game.
We can replace $\Diamond\ \gamma$ wth the fragments of LTL formulas
for which a deterministic generator can be easily computed~\cite{AlurT04}. 
%This methodology is described in details in this section.
\begin{algorithm}[t]
\begin{algorithmic}
\begin{tabbing}
\= Inputs : a system $S =(X,X_0,U,\rTo,Y,H)$, and \\
\> two LTL formulae $\varphi_{safe}$ and $\varphi_{guarantee}$\\
\> Output : System $P$\\
\> \\
\> 1. $\phi\ :=\ nnf(\lnot\varphi_{safe})$\\
\> \\
\> 2. $A^{Fine}_{\phi,nondet}$\ :=\ ConstructFineAutomata($Y,\phi$)\\
\> \\
\> 3. $A^{Fine}_{\phi}\ :=\ doSubsetConstruction(A^{Fine}_{\phi,nondet})$\\
\> \\
\> 4. $P_{\phi}\ :=\ computeSynchronousProduct(S,A^{Fine}_{\phi})$ \\
\> \\
\> 5. $P = SolveSafetyGame(P_{\phi},X \times (Q - F))$\\
\>\\
\> 6. {\bf if} ($\varphi_{guarantee} == \Diamond\ \gamma$)\\
\> \\
\> 7. \quad $P = SolveReachabilityGame(P,\gamma)$
\end{tabbing}
\end{algorithmic}
\caption{{\bf Synthesize($S, \varphi_{safe}, \varphi_{guarantee}$)}
\label{algo:synthesize}}
\end{algorithm}


%\paragraph{Syntax Checking and Splitting a Formula} The procedure $splitFormula(\varphi)$ checks whether the given LTL formula $\varphi$ belong to the subset of LTL grammer tool
%can handle. The procedure returns two subformulas of the given formula $\varphi_{safe}$
%and $\varphi_{live}$. These two formulas correspond to the safety and liveness counterpart
%of the given LTL formula respectively.
%For example, LTL formula $p\ \U\ q$ can be split into $(p\ \W\ q)$ and $\Diamond q$. 
%Similarly LTL formula
%$p\ U\ (q\ U\ r)$ can be split into two properties-$p\ W\ (q\ W\ r)$ and $\Diamond r$.
%A formula $(p\ W\ q) \land \Diamond r$ can be split into two formulas $p\ W\ q$ and $\Diamond r$.

%\paragraph{Compute NNF Form} For a given formula $\lnot\varphi_{safe}$, the negation
%normal form (NNF) of the formula is computed. The translation procedure works on the 
%syntax of the formula and pushes the negation operator from formulas to subformulas.
%For example, NNF form of the formula $\lnot (p\ \W\ q)$ is $(\lnot\ q) \U\ (\lnot p\ \land\ \lnot q)$

%
%
%
%\paragraph{Determinization by Subset Construction}
%%
%
%
%

%\paragraph{Symbolic Prefix Automata}
%The prefix automata is also encoded into symbolic representation. 
%
%
%\paragraph{Synchronous Product} The computation of synchronous product are performed
%symbolically.
%
%1. transition from the plant : $TR_{plant} (x,a,x')$\\
%2. labels: $L(x,p)$\\
%3. transition from specification : $TR_{spec} (q,p,q')$\\
%4. extended transition relation : $TR_{spec} $ 
%
%\paragraph{Solution of the safety game:} The solution of safety games are performed
%symbolically as well.
%
%\paragraph{Refinement}
%The computed controller needs to be refined to put into the concrete control loop.
%\paragraph{Controller synthesis for safe-LTL}

%
%\begin{figure}[htb]
%\begin{algorithm}{\bf computeSynchronousProduct(G,A)}
%\begin{algorithmic}
%\label{algo:product}
%\begin{tabbing}
%\= Inputs : a game $G =(X,X_p,X_a,X_0,U,\rTo,Y,H)$, and \\
%\> a fine automaton $A = (Q,Q_0,\delta,F)$\\
%\> Output : a game $P = (XQ,XQ_p,XQ_a,XQ_0,U,\rTo',Y,HQ)$\\
%\> \r{revise to make the notation consistent}\\
%\> 1. $XQ = X \times Q$\\
%\> 2, $XQ_0 = \{(x,q) \mid x \in X_0, \exists q_0 \in Q_0. q_0 \to_2^{L(x)} q'\} $,\\
%\> 3. $xq \to'^a x'q'$ if $x \to^a x' , q\to_2^{L(x')} q'$\\
%\> 4. $L(xq) = L(x)$ \\
%\end{tabbing}
%\end{algorithmic}
%\end{algorithm}
%\end{figure}
%\paragraph{Controller synthesis for Guarantee}
%We now consider the synthesis of controllers for a D-safe-LTL formula $\varphi$. As shown in Proposition~\ref{Prop:Decompose}, $\varphi$ can be decomposed as $\varphi=\psi\,\land\,\Diamond\, \gamma$ with $\psi$ and $\gamma$ safe-LTL formulas.

%\begin{figure}[htb]
%\begin{algorithm}{\bf solveLiveness($G,A,\Diamond r$)}
%\begin{algorithmic}
%\label{algo:product}
%\begin{tabbing}
%\= Inputs : a game $G =(X,X_p,X_a,X_0,U,\rTo,Y,H)$, \\
%\> a fine automaton $A = (Q,Q_0,\delta,F)$ and\\
%\> a live formula $\Diamond r$\\
%\> Output : Controller \\
%\> \r{revise to make the notation consistent}\\
%\> 1. $XQ = X \times Q$\\
%\> 2, $XQ_0 = \{(x,q) \mid x \in X_0, \exists q_0 \in Q_0. q_0 \to_2^{L(x)} q'\} $,\\
%\> 3. $xq \to'^a x'q'$ if $x \to^a x' , q\to_2^{L(x')} q'$\\
%\> 4. $L(xq) = L(x)$ \\
%\end{tabbing}
%\end{algorithmic}
%\end{algorithm}
%\end{figure}
%\section{Controller Synthesis}
%%We have applied the previous algorithms to the tool PESSOA.
%In this section, we assume that the symbolic abstraction of the continious system has been converted into a discrete system $S$.
%%The decomposition property in Proposition~\ref{Prop:Decompose} allows for a compositional approach to controller synthesis. 
%Algorithm~\ref{algo:synthesize} illustrates the steps we have implemented to construct the controller and the winning states of the plant $S$ with respect to the specification $\varphi_{safe}$ and $\varphi_{gurantee}$.
%Given two formulae $\varphi_{safe}$ and $\varphi_{gurantee}$, we can first compute the NNF of
%$\lnot \varphi_{safe}$ by calling \emph{nnf} procedure. 
%We have already described the algorithm for \emph{ConstructFineAutomata}.
%The constructed non-deterministic auomaton is determinized by the procedure \emph{doSubsetConstruction}.
%Given a deterministic fine automaton with respect to the $\lnot \varphi_{safe}$, and
%the system, the procedure \emph{computeSynchronousProduct} computes the product.
%The procedure $Solve$ $SafetyGame$ computes the winning set $W$ and the controller 
%transition relation $C$. The procedure also updates the winning states and transition relation of $P$ with the winning states $W$ and controller transition relation $C$ respectively.
%The guarantee requirement can be addressed afterwards by  \emph{SolveReachabilityGame}
%procedure on the synthesized safety controller. This methodology is described in details in this section.
%
%\begin{figure}[htb]
%\begin{algorithm}{\bf Synthesize($S, \varphi_{safe}, \varphi_{guarantee}$)}
%\begin{algorithmic}
%\label{algo:synthesize}
%\begin{tabbing}
%\= Inputs : a system $S =(X,X_0,U,\rTo,Y,H)$, and \\
%\> two LTL formulae $\varphi_{safe}$ and $\varphi_{guarantee}$\\
%\> Output : System $P$\\
%\> \\
%\> 1. $\phi\ :=\ nnf(\lnot\varphi_{safe})$\\
%\> \\
%\> 2. $A^{Fine}_{\phi,nondet}$\ :=\ ConstructFineAutomata($Y,\phi$)\\
%\> \\
%\> 3. $A^{Fine}_{\phi}\ :=\ doSubsetConstruction(A^{Fine}_{\phi,nondet})$\\
%\> \\
%\> 4. $P_{\phi}\ :=\ computeSynchronousProduct(S,A^{Fine}_{\phi})$ \\
%\> \\
%\> 5. $P = SolveSafetyGame(P_{\phi},X \times (Q - F))$\\
%\>\\
%\> 6. {\bf if} ($\varphi_{guarantee} == \Diamond r$)\\
%\> \\
%\> 7. \quad $P = SolveReachabilityGame(P,\Diamond r)$
%\end{tabbing}
%\end{algorithmic}
%\end{algorithm}
%\end{figure}
%
%
%%\paragraph{Syntax Checking and Splitting a Formula} The procedure $splitFormula(\varphi)$ checks whether the given LTL formula $\varphi$ belong to the subset of LTL grammer tool
%%can handle. The procedure returns two subformulas of the given formula $\varphi_{safe}$
%%and $\varphi_{live}$. These two formulas correspond to the safety and liveness counterpart
%%of the given LTL formula respectively.
%%For example, LTL formula $p\ \U\ q$ can be split into $(p\ \W\ q)$ and $\Diamond q$. 
%%Similarly LTL formula
%%$p\ U\ (q\ U\ r)$ can be split into two properties-$p\ W\ (q\ W\ r)$ and $\Diamond r$.
%%A formula $(p\ W\ q) \land \Diamond r$ can be split into two formulas $p\ W\ q$ and $\Diamond r$.
%
%%\paragraph{Compute NNF Form} For a given formula $\lnot\varphi_{safe}$, the negation
%%normal form (NNF) of the formula is computed. The translation procedure works on the 
%%syntax of the formula and pushes the negation operator from formulas to subformulas.
%%For example, NNF form of the formula $\lnot (p\ \W\ q)$ is $(\lnot\ q) \U\ (\lnot p\ \land\ \lnot q)$
%
%%
%%
%%
%%\paragraph{Determinization by Subset Construction}
%%%
%%
%%
%%
%
%%\paragraph{Symbolic Prefix Automata}
%%The prefix automata is also encoded into symbolic representation. 
%%
%%
%%\paragraph{Synchronous Product} The computation of synchronous product are performed
%%symbolically.
%%
%%1. transition from the plant : $TR_{plant} (x,a,x')$\\
%%2. labels: $L(x,p)$\\
%%3. transition from specification : $TR_{spec} (q,p,q')$\\
%%4. extended transition relation : $TR_{spec} $ 
%%
%%\paragraph{Solution of the safety game:} The solution of safety games are performed
%%symbolically as well.
%%
%%\paragraph{Refinement}
%%The computed controller needs to be refined to put into the concrete control loop.
%%\paragraph{Controller synthesis for safe-LTL}
%
%%
%%\begin{figure}[htb]
%%\begin{algorithm}{\bf computeSynchronousProduct(G,A)}
%%\begin{algorithmic}
%%\label{algo:product}
%%\begin{tabbing}
%%\= Inputs : a game $G =(X,X_p,X_a,X_0,U,\rTo,Y,H)$, and \\
%%\> a fine automaton $A = (Q,Q_0,\delta,F)$\\
%%\> Output : a game $P = (XQ,XQ_p,XQ_a,XQ_0,U,\rTo',Y,HQ)$\\
%%\> \r{revise to make the notation consistent}\\
%%\> 1. $XQ = X \times Q$\\
%%\> 2, $XQ_0 = \{(x,q) \mid x \in X_0, \exists q_0 \in Q_0. q_0 \to_2^{L(x)} q'\} $,\\
%%\> 3. $xq \to'^a x'q'$ if $x \to^a x' , q\to_2^{L(x')} q'$\\
%%\> 4. $L(xq) = L(x)$ \\
%%\end{tabbing}
%%\end{algorithmic}
%%\end{algorithm}
%%\end{figure}
%\paragraph{Controller synthesis for Reachability}
%%We now consider the synthesis of controllers for a D-safe-LTL formula $\varphi$. As shown in Proposition~\ref{Prop:Decompose}, $\varphi$ can be decomposed as $\varphi=\psi\,\land\,\Diamond\, \gamma$ with $\psi$ and $\gamma$ safe-LTL formulas.
% We first synthesize a controller $C_{\psi}$ enforcing $\psi$ on the system $S$ and consider the new system $C_{\psi}\times S$. Moreover, since $C_\psi$ is the least restrictive controller enforcing $\psi$, a controller enforcing $\varphi$ can now be obtained as $C_{\psi}\times C_{\Diamond\gamma}$ where $C_{\Diamond\gamma}$ is a controller enforcing $\Diamond\,\gamma$ on $C_{\psi}\times S$.
%The current implementation in {\sc pessoa} only handles formulas $\varphi=\psi\,\land\,\Diamond\,\gamma$ where $\gamma$ is an atomic proposition. Hence, the synthesis of a controller enforcing $\Diamond\,\gamma$ reduces to a simple reachability game with objective $\gamma$.
%\begin{figure}[htb]
%%\begin{algorithm}{\bf solveLiveness($G,A,\Diamond r$)}
%%\begin{algorithmic}
%%\label{algo:product}
%%\begin{tabbing}
%%\= Inputs : a game $G =(X,X_p,X_a,X_0,U,\rTo,Y,H)$, \\
%%\> a fine automaton $A = (Q,Q_0,\delta,F)$ and\\
%%\> a live formula $\Diamond r$\\
%%\> Output : Controller \\
%%\> \r{revise to make the notation consistent}\\
%%\> 1. $XQ = X \times Q$\\
%%\> 2, $XQ_0 = \{(x,q) \mid x \in X_0, \exists q_0 \in Q_0. q_0 \to_2^{L(x)} q'\} $,\\
%%\> 3. $xq \to'^a x'q'$ if $x \to^a x' , q\to_2^{L(x')} q'$\\
%%\> 4. $L(xq) = L(x)$ \\
%%\end{tabbing}
%%\end{algorithmic}
%%\end{algorithm}
%\end{figure}

